Progressive Multi-scale Fusion Network for RGB-D Salient Object Detection

Salient object detection(SOD) aims at locating the most significant object within a given image. In recent years, great progress has been made in applying SOD on many vision tasks. The depth map could provide additional spatial prior and boundary cues to boost the performance. Combining the depth information with image data obtained from standard visual cameras has been widely used in recent SOD works, however, introducing depth information in a suboptimal fusion strategy may have negative influence in the performance of SOD. In this paper, we discuss about the advantages of the so-called progressive multi-scale fusion method and propose a mask-guided feature aggregation module(MGFA). The proposed framework can effectively combine the two features of different modalities and, furthermore, alleviate the impact of erroneous depth features, which are inevitably caused by the variation of depth quality. We further introduce a mask-guided refinement module(MGRM) to complement the high-level semantic features and reduce the irrelevant features from multi-scale fusion, leading to an overall refinement of detection. Experiments on five challenging benchmarks demonstrate that the proposed method outperforms 11 state-of-the-art methods under different evaluation metrics.

==> egpaper_for_review.tex <==

\begin{document}

%%
%% The "title" command has an optional parameter,
%% allowing the author to define a "short title" to be used in page headers.
\title{Progressive Mask Guided Network for RGB-D Salient Object Detection  }

%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
\author{Guangyu Ren}
\authornote{Both authors contributed equally to this research.}
\email{g.ren19@imperial.ac.uk}
\orcid{1234-5678-9012}




%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
\renewcommand{\shortauthors}{Trovato and Tobin, et al.}

%%
%% The abstract is a short summary of the work to be presented in the
%% article.


%% A "teaser" image appears between the author and affiliation
%% information and the body of the document, and typically spans the
%% page.

%\begin{teaserfigure}

%\end{teaserfigure}
%%
%% This command processes the author and affiliation and title
%% information and builds the first part of the formatted document.
\maketitle

\section{Introduction}
Salient object detection(SOD) aims to detect the obvious and important objects in a given image. 
SOD is crucial for other vision tasks and has been applied in many different fields, such as semantic segmentation, scene classification, person re-identification, visual tracking and video summarization. 
The significance of SOD together with the rapid development of deep learning has led to substantial progress in recent years. However, there are still challenging issues on SOD, especially in complex scenarios which salient objects and background show similar appearance. 

Under this circumstance, depth maps\cite{lang2012depth} are introduced to provide complementary information to further enhance the detection performance in complex scenarios.


\newpage
\newpage










%%
%% If your work has an appendix, this is the place to put it.
\appendix

\section{Research Methods}


\end{document}
\endinput
%%
%% End of file `sample-authordraft.tex'.

